Introduction to Lattice QCD

These notes aim to provide a pedagogical introduction to Lattice QCD. The topics covered include the scope of LQCD calculations, lattice discretization of gauge and fermion (naive, Wilson, and staggered) actions, doubling problem, improved gauge and Dirac actions, confinement and strong coupling expansions, phase transitions in the lattice theory, lattice operators, a general discussion of statistical and systematic errors in simulations of LQCD, the analyses of the hadron spectrum, glueball masses, the strong coupling constant, and the quark masses.

==> Makefile <==
# %auto-ignore
MAINFILE=  main.tex

TEXFILES=  rgmac.latex title.tex LH.tex chap-intro.tex chap-connection.tex \
	   lqcd.tex chap-impglue.tex f-POT95lepage.tex \
	   chap-impdirac.tex chap-confine.tex \
	   chap-phase.tex chap-errors.tex chap-corr.tex \
	   chap-hm.tex chap-alpha.tex chap-mq.tex houch10.clo houches.cls

AXISFILES= f-wilsonloops.ax f-qqpotentialSU3.ax f-qqpotential.ax f-R0.ax \
	   f-rhofit.ax f-mbar.ax f-Wmbar.ax f-sigmalambda.ax f-pionmeff.ax \
	   f-nucleonmeff.ax f-rhomeff.ax f-hyperfine.ax f-GballsR0.ax

FIGFILES=  

PSFILES=   f-Bcontractions.eps f-Fp.eps f-QQCDpi.eps f-RTflow.eps f-etaprime.eps \
           f-fundadj.eps f-loop6ops.eps f-mfffig.eps f-pion.eps f-qqcd.eps \
	   f-rhopipi.eps f-strongcoupling.eps f_loopline.eps f_semileptonic1.eps \
	   CKM1.ps binding.ps f-baryfit.ps f-hmWILSON.ps f-nucfit.ps \
	   f_alphaworld.ps f-GBmorningstar.ps

#########################################################################
# special rules if any

#########################################################################
#									#
#                 NO USER SERVICEABLE PARTS BELOW !!!                   #
# 									#
#########################################################################


# List of all the sources
SOURCES= Makefile ${MAINFILE} ${TEXFILES} ${AXISFILES} ${FIGFILES} ${PSFILES}

# List of all postscript figures to be included.
PSINCLUSIONS= ${AXISFILES:.ax=.ps} ${FIGFILES:.fig=.ps} ${PSFILES}

# what is to be made by default
all: ${MAINFILE:.tex=.ps}

# re-dvips if any of these change
${MAINFILE:.tex=.ps}: ${MAINFILE:.tex=.dvi} ${PSINCLUSIONS}

# re-latex if any of these change
${MAINFILE:.tex=.dvi}: ${MAIN} ${TEXFILES} ${PSINCLUSIONS}

# Never try to `make' any of the sources
${SOURCES}:;

# The rest of them do not have any `extra' dependencies, i.e. a.x depends 
# obviously depends on a.y if a.x is to be created from a.y.

.PHONY: clean realclean
# clean removes ~ aux log and tmp files
clean:
	rm -f *~ *.aux *.log *.tmp
# real clean removes everything but sources and final products
realclean: clean
	rm -f ${AXISFILES:.ax=.ps} ${FIGFILES:.fig=.ps}

########################################################################
# General rules of how to build something from something else.
.SUFFIXES: .ps .dvi .tex .ax .xy .fig

# If .fig exists that is how to create ps.
%.ps: %.fig
	fig2dev -L ps $< > $@

# If .ax or .xy exist, that is the source of the .ps file
%.ps: %.ax
	xyplot $< | epsplot > $@.tmp
	sed -e "/%%BoundingBox: /d" -e '1a\
	'"`psbbox $@.tmp`" $@.tmp > $@ 
	rm -f $@.tmp
%.ps: %.xy
	xyplot $< | epsplot > $@.tmp
	sed -e "/%%BoundingBox: /d" -e '1a\
	'"`psbbox $@.tmp`" $@.tmp > $@ 
	rm -f $@.tmp

# else look for a dvi file.
%.ps: %.dvi
	dvips -z -o $@ $<


# dvi is always created from tex.
%.dvi: %.tex
	latex $<
	if grep -i -q rerun ${<:.tex=.log} ; then latex $<; fi
	if grep -i -q rerun ${<:.tex=.log} ; then latex $<; fi

##################################################################

submission: ${SOURCES} ${PSINCLUSIONS}
	tar cf submission.tar ${SOURCES} ${PSINCLUSIONS} && \
		(echo "."; echo "submission.tar"; echo "submission") | uufiles -gz -9 && \
		(sed -e 's/gunzip/tar xfz/' submission.uu > submission.tar) && \
		mv submission.tar submission.uu

